Large Language Models for Difficulty Estimation of Foreign Language Content with Application to Language Learning

We use large language models to aid learners enhance proficiency in a foreign language. This is accomplished by identifying content on topics that the user is interested in, and that closely align with the learner's proficiency level in that foreign language. Our work centers on French content, but our approach is readily transferable to other languages. Our solution offers several distinctive characteristics that differentiate it from existing language-learning solutions, such as, a) the discovery of content across topics that the learner cares about, thus increasing motivation, b) a more precise estimation of the linguistic difficulty of the content than traditional readability measures, and c) the availability of both textual and video-based content. The linguistic complexity of video content is derived from the video captions. It is our aspiration that such technology will enable learners to remain engaged in the language-learning process by continuously adapting the topics and the difficulty of the content to align with the learners' evolving interests and learning objectives.

==> bibliography.tex <==
@article{GPT,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya and others},
  year={2018},
  publisher={OpenAI}
}

@article{GPT3,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}

@article{palm,
  title="{Palm: Scaling language modeling with pathways}",
  author={Chowdhery, Aakanksha and Narang, Sharan and Devlin, Jacob and Bosma, Maarten and Mishra, Gaurav and Roberts, Adam and Barham, Paul and Chung, Hyung Won and Sutton, Charles and Gehrmann, Sebastian and others},
  journal={arXiv preprint arXiv:2204.02311},
  year={2022}
}

@article{llama,
  title={Llama: Open and efficient foundation language models},
  author={Touvron, Hugo and Lavril, Thibaut and Izacard, Gautier and Martinet, Xavier and Lachaux, Marie-Anne and Lacroix, Timoth{\'e}e and Rozi{\`e}re, Baptiste and Goyal, Naman and Hambro, Eric and Azhar, Faisal and others},
  journal={arXiv preprint arXiv:2302.13971},
  year={2023}
}

@article{koren2021advances,
  title={Advances in collaborative filtering},
  author={Koren, Yehuda and Rendle, Steffen and Bell, Robert},
  journal={Recommender systems handbook},
  pages={91--142},
  year={2021},
  publisher={Springer}
}

@article{transferLearning1,
  title={A survey of transfer learning},
  author={Weiss, Karl and Khoshgoftaar, Taghi M and Wang, DingDing},
  journal={Journal of Big data},
  volume={3},
  number={1},
  pages={1--40},
  year={2016},
  publisher={SpringerOpen}
}

@incollection{transferLearning2,
  title={Transfer learning},
  author={Torrey, Lisa and Shavlik, Jude},
  booktitle={Handbook of research on machine learning applications and trends: algorithms, methods, and techniques},
  pages={242--264},
  year={2010},
  publisher={IGI global}
}

@article{transferLearning3,
  title={A comprehensive survey on transfer learning},
  author={Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  journal={Proceedings of the IEEE},
  volume={109},
  number={1},
  pages={43--76},
  year={2020},
  publisher={IEEE}
}

@inproceedings{hernandez2022open,
  title={Open corpora and toolkit for assessing text readability in French},
  author={Hernandez, Nicolas and Oulbaz, Nabil and Faine, Tristan},
  booktitle={Proceedings of the 2nd Workshop on Tools and Resources to Empower People with REAding DIfficulties (READI) within the 13th Language Resources and Evaluation Conference},
  pages={54--61},
  year={2022}
}

@inproceedings{NEURIPS2020_1457c0d6,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {1877--1901},
 publisher = {Curran Associates, Inc.},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf},
 volume = {33},
 year = {2020}
}


@misc{bubeck_sparks_2023,
	title = {Sparks of {Artificial} {General} {Intelligence}: {Early} experiments with {GPT}-4},
	shorttitle = {Sparks of {Artificial} {General} {Intelligence}},
	url = {http://arxiv.org/abs/2303.12712},
	doi = {10.48550/arXiv.2303.12712},
	abstract = {Artificial intelligence (AI) researchers have been developing and refining large language models (LLMs) that exhibit remarkable capabilities across a variety of domains and tasks, challenging our understanding of learning and cognition. The latest model developed by OpenAI, GPT-4, was trained using an unprecedented scale of compute and data. In this paper, we report on our investigation of an early version of GPT-4, when it was still in active development by OpenAI. We contend that (this early version of) GPT-4 is part of a new cohort of LLMs (along with ChatGPT and Google's PaLM for example) that exhibit more general intelligence than previous AI models. We discuss the rising capabilities and implications of these models. We demonstrate that, beyond its mastery of language, GPT-4 can solve novel and difficult tasks that span mathematics, coding, vision, medicine, law, psychology and more, without needing any special prompting. Moreover, in all of these tasks, GPT-4's performance is strikingly close to human-level performance, and often vastly surpasses prior models such as ChatGPT. Given the breadth and depth of GPT-4's capabilities, we believe that it could reasonably be viewed as an early (yet still incomplete) version of an artificial general intelligence (AGI) system. In our exploration of GPT-4, we put special emphasis on discovering its limitations, and we discuss the challenges ahead for advancing towards deeper and more comprehensive versions of AGI, including the possible need for pursuing a new paradigm that moves beyond next-word prediction. We conclude with reflections on societal influences of the recent technological leap and future research directions.},
	urldate = {2023-04-12},
	publisher = {arXiv},
	author = {Bubeck, Sébastien and Chandrasekaran, Varun and Eldan, Ronen and Gehrke, Johannes and Horvitz, Eric and Kamar, Ece and Lee, Peter and Lee, Yin Tat and Li, Yuanzhi and Lundberg, Scott and Nori, Harsha and Palangi, Hamid and Ribeiro, Marco Tulio and Zhang, Yi},
	month = mar,
	year = {2023},
	note = {arXiv:2303.12712 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Artificial Intelligence},
}

@misc{openai_gpt-4_2023,
	title = {{GPT}-4 {Technical} {Report}},
	url = {http://arxiv.org/abs/2303.08774},
	doi = {10.48550/arXiv.2303.08774},
	abstract = {We report the development of GPT-4, a large-scale, multimodal model which can accept image and text inputs and produce text outputs. While less capable than humans in many real-world scenarios, GPT-4 exhibits human-level performance on various professional and academic benchmarks, including passing a simulated bar exam with a score around the top 10\% of test takers. GPT-4 is a Transformer-based model pre-trained to predict the next token in a document. The post-training alignment process results in improved performance on measures of factuality and adherence to desired behavior. A core component of this project was developing infrastructure and optimization methods that behave predictably across a wide range of scales. This allowed us to accurately predict some aspects of GPT-4's performance based on models trained with no more than 1/1,000th the compute of GPT-4.},
	urldate = {2023-04-12},
	publisher = {arXiv},
	author = {{OpenAI}},
	month = mar,
	year = {2023},
	note = {arXiv:2303.08774 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Artificial Intelligence},
}


@article{xia2019text,
  title={Text readability assessment for second language learners},
  author={Xia, Menglin and Kochmar, Ekaterina and Briscoe, Ted},
  journal={arXiv preprint arXiv:1906.07580},
  year={2019}
}

@phdthesis{tuncay2020app,
  title={App Attrition in Computer-Assisted Language Learning: Focus on Duolingo},
  author={Tuncay, Haluk Olcay},
  year={2020},
  school={McGill University (Canada)}
}

@inproceedings{liu2010personalized,
  title={Personalized news recommendation based on click behavior},
  author={Liu, Jiahui and Dolan, Peter and Pedersen, Elin R{\o}nby},
  booktitle={Proceedings of the 15th international conference on Intelligent user interfaces},
  pages={31--40},
  year={2010}
}


@article{habibi2015keyword,
  title={Keyword extraction and clustering for document recommendation in conversations},
  author={Habibi, Maryam and Popescu-Belis, Andrei},
  journal={IEEE/ACM Transactions on audio, speech, and language processing},
  volume={23},
  number={4},
  pages={746--759},
  year={2015},
  publisher={IEEE}
}

@inproceedings{zheng2018drn,
  title={DRN: A deep reinforcement learning framework for news recommendation},
  author={Zheng, Guanjie and Zhang, Fuzheng and Zheng, Zihan and Xiang, Yang and Yuan, Nicholas Jing and Xie, Xing and Li, Zhenhui},
  booktitle={Proceedings of the 2018 world wide web conference},
  pages={167--176},
  year={2018}
}

@inproceedings{guan2010document,
  title={Document recommendation in social tagging services},
  author={Guan, Ziyu and Wang, Can and Bu, Jiajun and Chen, Chun and Yang, Kun and Cai, Deng and He, Xiaofei},
  booktitle={Proceedings of the 19th international conference on World wide web},
  pages={391--400},
  year={2010}
}


@inproceedings{chen2016ctap,
  title={CTAP: A web-based tool supporting automatic complexity analysis},
  author={Chen, Xiaobin and Meurers, Detmar},
  booktitle={Proceedings of the workshop on computational linguistics for linguistic complexity (CL4LC)},
  pages={113--119},
  year={2016}
}
@article{mikolov2013word2vec,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}

@inproceedings{franccois2014analysis,
  title={An analysis of a french as a foreign language corpus for readability assessment},
  author={Fran{\c{c}}ois, Thomas},
  booktitle={Proceedings of the third workshop on NLP for computer-assisted language learning},
  pages={13--32},
  year={2014}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@inproceedings{okinina2020ctap,
  title={CTAP for Italian: Integrating components for the analysis of Italian into a multilingual linguistic complexity analysis tool},
  author={Okinina, Nadezda and Frey, Jennifer-Carmen and Weiss, Zarah},
  booktitle={Proceedings of the 12th Conference on Language Resources and Evaluation (LREC 2020},
  pages={7123--7131},
  year={2020}
}


@article{koenke1971another,
  title={Another practical note on readability formulas},
  author={Koenke, Karl},
  journal={Journal of Reading},
  volume={15},
  number={3},
  pages={203--208},
  year={1971},
  publisher={JSTOR}
}

@inproceedings{jiao-etal-2020-tinybert,
    title = "{T}iny{BERT}: Distilling {BERT} for Natural Language Understanding",
    author = "Jiao, Xiaoqi  and
      Yin, Yichun  and
      Shang, Lifeng  and
      Jiang, Xin  and
      Chen, Xiao  and
      Li, Linlin  and
      Wang, Fang  and
      Liu, Qun",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.372",
    doi = "10.18653/v1/2020.findings-emnlp.372",
    pages = "4163--4174",
    abstract = "Language model pre-training, such as BERT, has significantly improved the performances of many natural language processing tasks. However, pre-trained language models are usually computationally expensive, so it is difficult to efficiently execute them on resource-restricted devices. To accelerate inference and reduce model size while maintaining accuracy, we first propose a novel Transformer distillation method that is specially designed for knowledge distillation (KD) of the Transformer-based models. By leveraging this new KD method, the plenty of knowledge encoded in a large {``}teacher{''} BERT can be effectively transferred to a small {``}student{''} TinyBERT. Then, we introduce a new two-stage learning framework for TinyBERT, which performs Transformer distillation at both the pre-training and task-specific learning stages. This framework ensures that TinyBERT can capture the general-domain as well as the task-specific knowledge in BERT. TinyBERT4 with 4 layers is empirically effective and achieves more than 96.8{\%} the performance of its teacher BERT-Base on GLUE benchmark, while being 7.5x smaller and 9.4x faster on inference. TinyBERT4 is also significantly better than 4-layer state-of-the-art baselines on BERT distillation, with only {\textasciitilde}28{\%} parameters and {\textasciitilde}31{\%} inference time of them. Moreover, TinyBERT6 with 6 layers performs on-par with its teacher BERT-Base.",
}

@article{gou2021knowledge,
  title={Knowledge distillation: A survey},
  author={Gou, Jianping and Yu, Baosheng and Maybank, Stephen J and Tao, Dacheng},
  journal={International Journal of Computer Vision},
  volume={129},
  pages={1789--1819},
  year={2021},
  publisher={Springer}
}

@inproceedings{martin-etal-2020-camembert,
    title = "{C}amem{BERT}: a Tasty {F}rench Language Model",
    author = "Martin, Louis  and
      Muller, Benjamin  and
      Ortiz Su{\'a}rez, Pedro Javier  and
      Dupont, Yoann  and
      Romary, Laurent  and
      de la Clergerie, {\'E}ric  and
      Seddah, Djam{\'e}  and
      Sagot, Beno{\^\i}t",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/2020.acl-main.645",
    pages = "7203--7219",
    abstract = "Pretrained language models are now ubiquitous in Natural Language Processing. Despite their success, most available models have either been trained on English data or on the concatenation of data in multiple languages. This makes practical use of such models {--}in all languages except English{--} very limited. In this paper, we investigate the feasibility of training monolingual Transformer-based language models for other languages, taking French as an example and evaluating our language models on part-of-speech tagging, dependency parsing, named entity recognition and natural language inference tasks. We show that the use of web crawled data is preferable to the use of Wikipedia data. More surprisingly, we show that a relatively small web crawled dataset (4GB) leads to results that are as good as those obtained using larger datasets (130+GB). Our best performing model CamemBERT reaches or improves the state of the art in all four downstream tasks.",
}

@inproceedings{Bert2019,
  author       = {Jacob Devlin and
                  Ming{-}Wei Chang and
                  Kenton Lee and
                  Kristina Toutanova},
  editor       = {Jill Burstein and
                  Christy Doran and
                  Thamar Solorio},
  title        = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
                  Understanding},
  booktitle    = {Proceedings of the 2019 Conference of the North American Chapter of
                  the Association for Computational Linguistics: Human Language Technologies,
                  {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
                  and Short Papers)},
  pages        = {4171--4186},
  publisher    = {Association for Computational Linguistics},
  year         = {2019},
  url          = {https://doi.org/10.18653/v1/n19-1423},
  doi          = {10.18653/v1/n19-1423},
  timestamp    = {Mon, 26 Sep 2022 12:21:55 +0200},
  biburl       = {https://dblp.org/rec/conf/naacl/DevlinCLT19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{deepsparse,
  
  author = {Shen, Haihao and Zafrir, Ofir and Dong, Bo and Meng, Hengyu and Ye, Xinyu and Wang, Zhe and Ding, Yi and Chang, Hanwen and Boudoukh, Guy and Wasserblat, Moshe},
  
  keywords = {Computation and Language (cs.CL), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Fast DistilBERT on CPUs},
  
  journal = {arXiv preprint arXiv:2211.07715},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@inproceedings{opencorporaFrench2022,
  title="{Open corpora and toolkit for assessing text readability in French}",
  author={Hernandez, Nicolas and Oulbaz, Nabil and Faine, Tristan},
  booktitle={Proceedings of the 2nd Workshop on Tools and Resources to Empower People with REAding DIfficulties (READI) within the 13th Language Resources and Evaluation Conference},
  pages={54--61},
  year={2022}
}

@article{yin2019benchmarking,
  title={Benchmarking zero-shot text classification: Datasets, evaluation and entailment approach},
  author={Yin, Wenpeng and Hay, Jamaal and Roth, Dan},
  journal={arXiv preprint arXiv:1909.00161},
  year={2019}
}

@article{wesely2010student,
  title={Student attrition from traditional and immersion foreign language programs},
  author={Wesely, Pamela M},
  journal={Language and Linguistics Compass},
  volume={4},
  number={9},
  pages={804--817},
  year={2010},
  publisher={Wiley Online Library}
}

@article{maley2005,
title = {Extensive Reading Activities for the Second Language Classroom},
author = {Maley, A},
year = "2005",
journal = {ELT Journal, 59(4)},
pages = {354 -- 355}
}

@article{prowse2002top,
  title={Top ten principles for teaching extensive reading: A response},
  author={Prowse, Philip},
  year={2002},
  journal={University of Hawaii National Foreign Language Resource Center}
}


@inproceedings{Lungu18,
  author = {Mircea Filip Lungu and Luc van den Brand and Dan Chirtoaca and Martin Avagyan},
  title = {As We May Study: Towards the Web as a Personalized Language Textbook}, 
  booktitle = {Proc. of CHI}, 
  pages = {338}, 
  year = {2018}, 
  biburl = {https://dblp.org/rec/bib/conf/chi/LunguBCA18}, 
  bibsource = {dblp computer science bibliography, 
  https://dblp.org} }


@book{krashen2004power,
  title={The power of reading: Insights from the research: Insights from the research},
  author={Krashen, Stephen D},
  year={2004},
  publisher={ABC-CLIO}
}
@article{burnette2016renewal,
  title={The renewal of competency-based education: A review of the literature},
  author={Burnette, Diane M},
  journal={The Journal of Continuing Higher Education},
  volume={64},
  number={2},
  pages={84--93},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{book2014all,
  title={All Hands on Deck: Ten Lessons from Early Adopters of Competency-Based Education.},
  author={Book, Patricia A},
  journal={Western Interstate Commission for Higher Education},
  year={2014},
  publisher={ERIC}
}
@inproceedings{franccois2012ai,
  title={An “AI readability” formula for French as a foreign language},
  author={Fran{\c{c}}ois, Thomas and Fairon, C{\'e}drick},
  booktitle={Proceedings of the 2012 joint conference on empirical methods in natural language processing and computational natural language learning},
  pages={466--477},
  year={2012}
}

@book{boss2022reinventing,
  title={Reinventing project-based learning: Your field guide to real-world projects in the digital age},
  author={Boss, Suzie and Krauss, Jane},
  year={2022},
  publisher={International Society for Technology in Education}
}

@book{atwell2015middle,
  title={In the middle: A lifetime of learning about writing, reading, and adolescents},
  author={Atwell, Nancie},
  year={2015},
  publisher={Heinemann}
}

@article{daybamford2002,
  title={Top ten principles for teaching extensive reading},
  author={Day, Richard and Bamford, Julian},
  year={2002},
  publisher={University of Hawaii National Foreign Language Resource Center}
}

@ARTICLE{10.3389/fnhum.2018.00305,
  
AUTHOR={Klimova, Blanka},   
	 
TITLE={Learning a Foreign Language: A Review on Recent Findings About Its Effect on the Enhancement of Cognitive Functions Among Healthy Older Individuals},      
	
JOURNAL={Frontiers in Human Neuroscience},      
	
VOLUME={12},           
	
YEAR={2018},                
	
ISSN={1662-5161},   
   
ABSTRACT={Currently, there is an increasing number of older population groups, especially in developed countries. This demographic trend, however, may cause serious problems, such as an increase in aging diseases, one of which is dementia whose main symptom consists in the decline of cognitive functioning. Although there has been ongoing pharmacological research on this neurological disorder, it has not brought satisfying results as far as its treatment is concerned. Therefore, governments all over the world are trying to develop alternative, non-pharmacological strategies/activities, which could help to prevent this cognitive decline while this aging population is still healthy in order to reduce future economic and social burden. One of the non-pharmacological approaches, which may enhance cognitive abilities and protect against the decline in healthy older population, seems to be the learning of a foreign language. The purpose of this mini-review article is to discuss recent findings about the effect of foreign language learning on the enhancement of cognitive functions among healthy older individuals. The findings, divided into three research areas, show that the learning of a foreign language may generate a lot of benefits for older individuals, such as enhancement of cognitive functioning, their self-esteem, increased opportunities of socializing, or reduction of costs. However, as Ware et al. (<xref ref-type="bibr" rid="B49">2017</xref>) indicate, any intervention program on foreign language learning should be well thought of and tailored to the needs of older people in order to be effective and avoid accompanying factors, such as older people’s anxiety or low self-confidence. Nevertheless, more empirical studies should be done in this area.}
}

@article{imperial2021bert,
  title={Bert embeddings for automatic readability assessment},
  author={Imperial, Joseph Marvin},
  journal={arXiv preprint arXiv:2106.07935},
  year={2021}
}

@inproceedings{wilkens2022fabra,
  title={Fabra: French aggregator-based readability assessment toolkit},
  author={Wilkens, Rodrigo and Alfter, David and Wang, Xiaoou and Pintard, Alice and Tack, Ana{\"\i}s and Yancey, Kevin P and Fran{\c{c}}ois, Thomas},
  booktitle={Proceedings of the Thirteenth Language Resources and Evaluation Conference},
  pages={1217--1233},
  year={2022}
}

@article{lee2022editable,
  title={An editable learner model for text recommendation for language learning},
  author={Lee, John SY},
  journal={ReCALL},
  volume={34},
  number={1},
  pages={51--65},
  year={2022},
  publisher={Cambridge University Press}
}

@misc{krashen2003explorations,
  title={Explorations in language acquisition and use},
  author={Krashen, Stephen D},
  year={2003},
  publisher={Heinemann Portsmouth, NH}
}

@article{jeon2021exploring,
  title={Exploring AI chatbot affordances in the EFL classroom: Young learners’ experiences and perspectives},
  author={Jeon, Jaeho},
  journal={Computer Assisted Language Learning},
  pages={1--26},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{lin2021learning,
  title={Learning analytics for investigating the mind map-guided AI chatbot approach in an EFL flipped speaking classroom},
  author={Lin, Chi-Jen and Mubarok, Husni},
  journal={Educational Technology \& Society},
  volume={24},
  number={4},
  pages={16--35},
  year={2021},
  publisher={JSTOR}
}

@article{underwood2017exploring,
  title={Exploring AI language assistants with primary EFL students},
  author={Underwood, Joshua},
  journal={CALL in a climate of change: adapting to turbulent global conditions--short papers from EUROCALL},
  volume={2017},
  pages={317--321},
  year={2017}
}

@article{dizon2020evaluating,
  title={Evaluating intelligent personal assistants for L2 listening and speaking development},
  author={Dizon, Gilbert},
  year={2020},
  publisher={University of Hawaii National Foreign Language Resource Center}
}



@article{moussalli2020intelligent,
  title={Intelligent personal assistants: can they understand and be understood by accented L2 learners?},
  author={Moussalli, Souheila and Cardoso, Walcir},
  journal={Computer Assisted Language Learning},
  volume={33},
  number={8},
  pages={865--890},
  year={2020},
  publisher={Taylor \& Francis}
}
